The role of formalism in system requirements (full version)

A major determinant of the quality of software systems is the quality of their requirements, which should be both understandable and precise. Most requirements are written in natural language, good for understandability but lacking in precision. To make requirements precise, researchers have for years advocated the use of mathematics-based notations and methods, known as "formal". Many exist, differing in their style, scope and applicability. The present survey discusses some of the main formal approaches and compares them to informal methods. The analysis uses a set of 9 complementary criteria, such as level of abstraction, tool availability, traceability support. It classifies the approaches into five categories: general-purpose, natural-language, graph/automata, other mathematical notations, seamless (programming-language-based). It presents approaches in all of these categories, altogether 22 different ones, including for example SysML, Relax, Eiffel, Event-B, Alloy. The review discusses a number of open questions, including seamlessness, the role of tools and education, and how to make industrial applications benefit more from the contributions of formal approaches. (This is the full version of the survey, including some sections and two appendices which, because of length restrictions, do not appear in the submitted version.)

==> notes/multiviews.tex <==
\section{FORMOSE}
\label{sec:formose}

In \cite{golra_addressing_2016} the authors propose a new method to make the link between specifications expressed in several ways. Indeed, contrary to traditional \gls{MDE} approach that propose to use models transformations to change from a model to another, they propose a "space" vision. Stakeholders models can be seen as technical spaces, used to express specific needs of a domain, and to compose several subsystems in a common one, a conceptual space is used to make the link between interfaces of different domains.

They so mapped concepts expressed with several paradigms (EMF, XML, Word documents, etc) in a common interface. If a stakeholder chooses to change their specification, the common system will be impacted but, contrary to model transformation approach, other stakeholders will not have to transform models again. They provides open source tools to their methods, grouped in the openflexo project\footnote{https://www.openflexo.org/}.

In \cite{golra_continuous_2016}, the same authors propose to apply their model federation principle to requirements, considering the different ways to express requirements as technological space and linking them in the conceptual space. It permits to link requirements expressed in a Word Document for example to other requirements expressed in the KAOS approach.

These works seems very promising. Indeed, the use of a central interface language, their conceptual space, facilitate the translucence between several stakeholders. Their model transformation mechanism so permit to easily measure the impact of a change in a paradigm in the others. However, it is needed to implement several technological connectors to bridge the gap between their virtual models and the technological spaces. Thus, if a technological connector does not exists, the writing of such connector is needed and, even if it exists an open-source tool, there is a need for a software expert to implement it.
In our opinion, a way to overcome this issue is to provide a language that can be understanding by non-software engineers and that can be used to write transformation from \gls{DSML} to this interface. Another research lead can be to explore automatic models transformations to deduce technological connectors.

\section{GEMOC}


==> notes/req-express.tex <==
The need for a more formal expression of requirements exists in requirements engineering between several decades. Indeed, due to the fact that the main way to express requirements was -- and still is -- the natural language, researchers try to propose tools to help the requirements analysis.

However, most of the works are focusing on the need to express relationship between requirements or on the different way to classified requirements, from goals to non functional requirements. Thus, in \cite{ceron_meta-model_2005}, the authors propose a metamodel to express relationship between requirements themselves and between requirements and other artifacts of the system, such as use case that should describe a functional requirements and lead to discover new features. The issue of such approaches is that still require an human to express the semantic induced by requirements.

In our opinion, the formalization of requirements now must focus on this need of semantic to allow a better automation of requirements analysis, in order to let machine deduce links that are trivial, while experts will focus on more complex stuff.

\section{\gls{URML}}

In \cite{berenbach_use_2012}, the authors propose a modeling language for requirements (\gls{URML} \cite{helming_towards_2010}) in order to overcome several issue encountered by industrials partners. They propose a \gls{UML} profile for requirements and notions that are, according to them, linked to this requirements (e.g., threats, hazards and mitigations or even product lines). They also propose a concrete syntax with a only notational element for every element of metamodel.

This approach thus propose to add some semantic on links between requirements and other artifacts, and, regarding to \gls{SysML} requirements -- another \gls{UML} profile --, the introduction of danger notions allow to justify the need of some requirements. However, even if this language is a \gls{UML} profile, the integration of \gls{URML} to existing tools could be discussed -- especially since we know that this is a main issue in acceptation on new approach. Moreover, in their work the authors focused on the existing relationship between requirements and other elements, not on the way to express requirements -- even if requirements can be linked to use case or process to try to introduce this notion. 

\section{On the {Use} of {Domain} and {System} {Knowledge} {Modeling} in {Goal}-{Based} {Event}-{B} {Specifications} \cite{mammar_use_2016}}

In this paper, the authors propose an approach to express with the Event-B method a system and requirements from \gls{GORE} KAOS. Indeed, their approach aims to link requirements and the system in the Event-B method by two "approaches:
\begin{itemize}
  \item expression of requirements that are formalized as Event-B logical expressions;
  \item representation of the system itself, describe with ontology derived from object representation of system.
\end{itemize}

The first of these two approaches is detailed in \cite{matoussi_event-b_2010}. It consists as a description of the initial formal specification, extracting relations between requirements deduced on their relations in KAOS --- especially composition links of KAOS can be expressed as a logical \texttt{AND} between requirements of the composition.

In \cite{mammar_use_2016}, the authors are more precisely describing the system itself, in order to link requirements with the specification. The objective of this paper is inter alia to insert this formal specification into the FORMOSE OpenFlexo project (more detailed in \ref{sec:formose}). The authors describe an approach to create a technological connector for this formal representation.

Thus, this work aims to link requirements to specification, in a kind of multirequirements approach. The use of a formal syntax for requirements and links between requirements can lead user to prove the correctness of system and, moreover, to validate the system --- you can prove that system respect requirements expressed by stakeholders. 
However, this approach still require an expert to refine requirements in the B language. In our opinion, a major issue that cause low acceptance of new approaches is the difficulty of new tools. The OpenFlexo system is a potential solution to this gap, allowing stakeholders to describe requirements in their favorite paradigm and to then linked them to a more formal like this one.
The intervention of an expert can then lead to a system proof, that can be useful in a certification process for example.
Nevertheless, we think that an approach a bit less formal but automatic can lead requirements engineers to detect in an upstream phase problems of system, without the need of a proof expert. 

\section{Syntactic and semantic definition of requirements}

Most of works on requirements formalization are treating about the need to enrich a traditional \emph{identifier + text} representation with notions such as priority or risk \cite{soares_user_2011}. In \cite{albinet_memvatex_2008}, Albinet et al. introduce notions of source reference and justification in requirements; these two additions thus allows a better traceability to upstream phase. However, if this kind of representation can be sufficient for non-functional requirements, in our opinion we can go a step further with functional ones.

Indeed, functional requirements are often formalized in \gls{MDE} with data flow diagram or use case diagram \cite{dahan_comparing_2014}. Metamodels of these diagrams can thus be used as a grammar for requirements, providing a syntactic formalization. Nevertheless, a use case can (and must) be refined with other concepts and remains a natural language sentence, although better structured than requirements expressed in pure natural language.

In \cite{scott_context-free_2004}, the authors propose a grammar for requirements expressed in a constrained natural language. They provide a syntax to lead the expression of requirements during elicitation, allowing the capture of constituent components of requirements. Rules can then be applied to these components to detect issues (e.g., an acceptance limit should be a number). However, concepts thus captured are semantically defined by there lexical classes. Therefore, two nouns are not semantically differentiated and still need a domain expert to define the semantic of these concepts. In our opinion, this is a major issue of this work and we hope that a \gls{MDE} approach can lead us to provide these semantic.

A research track for this semantic can be found in \cite{dzung_improvement_2009}. In this paper, Dzung and Ohnishi propose to parse requirements to match them with ontologies of the domain, applying a set of rules to check and deduce relationship between requirements. In this work, the authors only treat the requirements elicitation phase and provide tools to ease this step; they do not treat traceability to downstream phase. However, they propose a metamodel (see fig. \ref{fig:mm-req}) for requirements, based on relationship between requirements, and different concepts that composed them (who, where, why, when). A mapping of these concepts with objects of the domain can then be proposed to analyze requirements.

\begin{figure}
  \centering
  \includegraphics{img/mm-req}
  \caption{\label{fig:mm-req}Metamodel of requirements ontology from \cite{dzung_improvement_2009}}
\end{figure}

\section{Translation from natural language requirements to a more formal representation}

In \cite{aceituna_evaluating_2011}, the authors proposed an approach to incrementally translate natural language requirements in state transition diagram. In their opinion, functional requirements can be expressed as a transition from a state to another. They so try to create a triplet composed by two states and a transition. However; due to the ambiguity of natural language, some of the requirements cannot be totally translated. This is why there approach is incremental; expert are still required to check and complete produced state transition diagrams.

Even if this approach allows users to express requirements in a natural language way and to translate it in a more formal way, it cannot be totally be automated due to the natural language. This issue cannot be overcame, this is why, in our opinion, we should restrict the natural language to a constrained subset -- a \gls{DSL} -- that can be more easily automated.

\section{Quality of requirements}

Several modeling languages for requirements have been proposed in literature; we presented some of them. Nowadays, the more used tools still are tools that are working with natural language, like \emph{IBM Rational Doors} or \gls{GORE} approaches. In \cite{soares_user_2011}, the authors proposed a set of properties for good a user requirements language and classified some existing requirements languages according to these properties. Among these qualities, they espcially mentioned the availability of graphical modeling, the human readability, the relationship between requirements, the relationship between requirements and design and, to a lesser extent, the machine readability and a well-defined semantics.

These two last properties may be less important for user requirements, but in our opinion, if we want to help as much as possible the treatment of requirements in the following steps, there are crucial.

% Rewrite table based on article of Soares
\begin{table}
  \caption{}
  \label{tab:}

  \begin{center}
    \begin{tabular}{|c|c|c|c|c|c||c|c|}
      \multicolumn{1}{c}{} & \multicolumn{1}{c}{\rotatebox{75}{Single model principle}} &
                             \multicolumn{1}{c}{\rotatebox{75}{Multiviews}} & 
                             \multicolumn{1}{c}{\rotatebox{75}{Human-readable}} & 
                             \multicolumn{1}{c}{\rotatebox{75}{Interpretable}} & 
                             \multicolumn{1}{c}{\rotatebox{75}{Formal}} & 
                             \multicolumn{1}{c}{\rotatebox{75}{Software Engineering}} & 
                             \multicolumn{1}{c}{\rotatebox{75}{System Engineering}} \\
       \hline
       Multirequirements & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark \\
       \hline
       Formose & $\pm$ & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
       \hline
       SysML & $\pm$ & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark \\
       \hline
       IBM Rational DOORS & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark \\
       \hline
       RELAX & \xmark & \xmark & $\pm$ & \cmark & \cmark & \xmark & \cmark \\
       \hline
       FORM-L & \xmark & \xmark & $\pm$ & \cmark & \cmark & \xmark & \cmark \\
       \hline
       Requirements Grammar & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark \\
       \hline
       fSysML & \cmark & $\pm$ & $\pm$ & \xmark & \cmark & \xmark & \cmark \\
       \hline
        KAOS to UML/OCL & \xmark & \cmark & \cmark & $\pm$ & \cmark & \cmark & \xmark \\
       \hline
        & & & & & & & \\
       \hline
    \end{tabular}
  \end{center}
\end{table}


==> notes/thesis-plan-content.tex <==
\section{Summary}

Seamless development aims to link different phases of the software development life cycle, from design to implementation. In software engineering, this is an effective way to prevent bugs \cite{broy_seamless_2010}. In system engineering, there is a need to apply the same kind of technique, requirements can be critical. The main objective of the thesis is to contribute to this effort in the specific requirement engineering activity because this phase is crucial in each the following steps of a project. We will focus on traceability links between different artifacts of specifications and implementations. The expected contributions are:
\begin{itemize}
  \item definition of an abstraction of requirements that would be used as an artifact as such, in a compatible representation with other artifacts of specification;
  \item definition of a formal notation for requirements in order to be able to assess the system validity throughout the design and development;
  \item definition of a bi-directional relationship between requirements and artifacts so that are can be converted into the other.
\end{itemize}
The main goal is so to introduce some formalism in requirements' expression, in order to detect design failures. Engineering complex systems usually involve several stakeholders; we also need to keep some flexibility in order to be able to treat different domains. We so aim to introduce a kind of translucence between requirements expressed in several stages of development and from several domains.

\section{Introduction}

Complex systems design implies several stakeholders, from different domains. Due to this skills' heterogeneity, the specification of these systems is done with several different artifacts (e.g., text documents, requirements database, \gls{SysML} diagrams, etc.). To ensure final product quality, one of the main challenges of system engineering is to be able to link these different artifacts.

Indeed, it still exists a coherence lack between the several views --- the different artifacts used to specify the system.
Using these views unrelated makes harder inconsistency detection, like conflicting requirements.
A multiviews approach, with a dedicated unique language or with a common abstraction of specifications' artifacts would allow to detect the inconsistency upstream. \\

It also exists a traceability problem with design and system realization. Indeed, the lack of clear correlation between system implementation and requirements does not allow to totally compute changes' consequences. Multirequirements \cite{meyer_multirequirements_2013} aims to interweave specifications and development, in order to reduce the gap between requirements and system implementation in a seamless purpose. The introduction of multi-requirements' concept would then permit to make the link between several levels of abstraction, in order to compute change impact.

Moreover, using a common language for specification and conception would lead us to reintroduce into system the requirements deduced from system implementation.\\

\gls{MBSE}, which is increasingly used in system engineering, proposes an approach that uses models as central artifact. Modeling provides a possible way to define a common interface between different views and abstractions. \\

The main goal of this thesis is to define methods and tools for these "multi" approaches. One of the expected contributions is the use of \gls{MBSE} in order to provide a way to express requirements that would be used as common interface between artifacts.

Rather than to propose the use of a unique language as a way to express requirements --- proposition made harder by force of habits and the number of different stakeholders, implying the creation to a human-readable language, accessible to everybody ---, we think that the use of a common modeling language would permit us to make the link (as show fig. \ref{fig:multiple-to-common}), while allowing engineers to use their usual tools. \\

\begin{figure}[h]
  \centering
  \includegraphics[scale=0.6]{img/multiple-to-common.pdf}
  \caption{\label{fig:multiple-to-common}Using a common language as interface between several domains languages}
\end{figure}

Another expected contribution is the introduction of a formalism in the requirement expression, with a constraint language, in order to detect inconsistency in systems.

The \emph{\gls{OCL}} is a language used to enrich \gls{UML} models, by adding invariants constraints. By so, it is a potential candidate for this formalization, allowing us to constrain links between artifacts or even artifacts' element values. However, more applicative languages, such as \emph{Eiffel}, can permit us to take advantages of a formal language and to make the link with the multirequirements approach.

Indeed, another goal of this thesis is to provide a way to express specification and realization in a same formalism, to avoid the gap between these different abstractions. Using an object-oriented programming language would so be a way to use the \gls{MBSE} approach, while allowing an execution for simulation or validation purpose. Thus, Eiffel would permits, with object-oriented and design by contracts paradigms, to link applicative and constraints aspects.

\section{State-of-the-Art}

\subsection{Expression of requirements}
\label{sec:requirements_expression}

The use of a dedicated language to express requirements has been studied on several occasions. 

There are a number of industrial solutions \cite{gea_requirements_2011}, like \emph{IBM Rational DOORS}\footnote{http://www-03.ibm.com/software/products/en/ratidoor} or \emph{Dassault Systems' Reqtify}\footnote{http://www.3ds.com/products-services/catia/products/reqtify/}, that nowadays exist and provide tools to manage requirements in complex systems. These solutions let users make relation between requirements expressed in several ways to introduce traceability into the systems. For example, in Reqtify, you can import requirements expressed in a Microsoft Word document and link them to some C code that implement these specifications. These tools also provide ways to make link from requirements, from different stages or in the same. However, and regardless to their proprietary formats, these tools does not provide a strong semantic on links. Furthermore, requirements are expressed in natural language and without particular syntax, that can make difficult to deduce links.

\gls{SysML} \cite{object_management_group_omg_omg_2007} provides a diagram type to express requirements --- requirement diagram --- that leads to incorporate the specification into the modeling process. While the standard use case diagrams can lead user to express functional requirements, this new type of diagram permits user to express functional and non-functional requirements (as an element with text) and to define relationship between requirements and other diagrams elements (like blocks, uses cases or even other requirements). \gls{SysML} does not have the possibility to link requirements expressed with other languages, unlike the previously presented tools, but the PolarSys\footnote{https://www.polarsys.org/} development tool for complex systems provides a plugin, named ReqCycle\footnote{https://www.polarsys.org/projects/polarsys.reqcycle}, that can reference other specification documents.

So tools introduce the notion of traceability between artifacts. Nevertheless, they mostly work only with textual requirements. In the more advanced of them, it is possible to link artifacts with concrete documents.

To overcome this expression difficulty, some works try to impose a syntax to express requirements. In \cite{whittle_relax:_2009}, the authors propose a language to express requirements in a \gls{CAS} context. For this, Witthle et al. present a structured natural language, named \textsc{Relax}, that permits to specify requirements with some of them that can be relaxed, in order to keep safe priority requirements of the \gls{CAS}.
Recently, \cite{nguyen_verification_2015} proposed an extension for the Modelica \cite{mattsson_physical_1998} modeling language, named \emph{FORM-L}, to allow formal modeling of requirements. These languages are designed to be addressed to stakeholders. However, these approaches implie to stakeholders to learn these new syntaxes and to abandon their traditional tools. Furthermore, these works were developped for topical domains and thus are very specific \glspl{DSL}.

Thus, the use of a common language is steel needed to provide a way to link different artifacts. The \gls{INCOSE} in the Vision 2025 document \cite{incose_se_????} is especially treating about the need to conciliate the multiple stakeholder viewpoints. The \gls{GEMOC} initiative \cite{combemale_globalizing_2014} aims to provide a common interface for different \glspl{DSML}, used to express the needs specific to different stakeholders; they propose to use models as base artifacts to bridge the gap between \glspl{DSL}, in the same way that \gls{MDE} uses models as a central artifact between specification and implementation. Moreover, the acceptance of this approach can be eased by the growth of interest of \gls{MBSE} in system engineering industry.  

A \gls{MBSE} approach would be to express requirements as modeling elements as precisely as other modeling artifacts. This approach can lead us to create links between requirements and other modeling artifacts from several stakeholders. Thus, we can combine elements from several domains in a holistic view, taking into account link between domain specific artifacts and also between these artifacts and requirements.

\subsection{Requirements formalization}

The need for consistency in requirements expressed in the IEEE standard 830-1993 \cite{committee_ieee_1998} is a crucial point in the specification validation. The formalization of requirements should lead us to computerize this validation; indeed, if we are able to express requirements in a semantic defined language, the formal logic can be used to find non-valid expression.

The \textsc{Relax} language mentioned in section \ref{sec:requirements_expression} is semantically defined with fuzzy branching temporal logic \cite{moon_fuzzy_2004}. Thus, this semantic can be used as a validation basis through the benefit of validation tools.

However, some other research leads are interesting; indeed, due to the fact that requirements can be see as "contracts" between the client and the supplier, the design by contracts can be considered as a way to formalize requirements.
The main idea of design by contracts \cite{meyer_applying_1992} in software programming is to introduce notions of preconditions (a routine requirements), postconditions (properties ensured after a routine's execution) and invariants (logical expression always true) in an object-oriented context. In that way, making explicit declarations of contracts allows users to avoid some unwanted behaviors by checking the validity of these conditions.

The \gls{OCL} \cite{object_management_group_omg_ocl_2014} is a formal language that provides a way to express constraints on \gls{UML} \cite{object_management_group_omg_uml_2015} models. In \cite{hahnle_authoring_2002}, Hähnle et al. propose an interface between a subset of the English natural language and \gls{OCL}; this work can be seen as a way to formalize requirements (here constraints) in a better semantically defined language. This approach allows to help the user to express constraints of the system in a more human-readable way while maintaining enough formalism to analyze the system (here, check if models are conforms to constraints). An example for a \verb$Queue$ class is given in fig. \ref{fig:ocl-eng}; preconditions and postconditions of \verb$Queue::getFirst()$ operation can be expressed both in English and OCL, and are automatically translate in the other language. 

\begin{figure}[h!]
\begin{description}
  \item[Operation] getFirst 
  \item[OCL:] \begin{verbatim}
context Queue::getFirst() : Integer
pre:  self.size() > 0
post: result = self.asSequence()->first
\end{verbatim}
  \item[English:] for the operation getFirst() : Integer of the class Queue, the following precondition should hold: \\
  \hspace*{2ex} the size of the queue is greater than zero \\
  and the following postcondition should hold: \\
  \hspace*{2ex} the result is equal to the first element of the queue
\end{description}
\caption{\label{fig:ocl-eng}Example from \cite{hahnle_authoring_2002} of a matching between English and OCL}
\end{figure}
Another way to express constraint in a system is with \gls{CSP}, that allows to define three sets (variables, domains of variables and constraints) that can be used by a \gls{CSP} solver \cite{merchez_abscon:_2001} to instantiate variables with values from their domains conform to constraints. Several works already exist \cite{ferdjoukh_instantiation_2015} in models' modeling as a \gls{CSP}, and we want to explore the translation of requirements into a CSP.

In \cite{meyer_multirequirements_2013}, Meyer proposes an approach to express requirement directly inside the Eiffel source code, using especially Eiffel's contracts as a way to express requirements. The formalism of these contracts can lead user, with tools like AutoProof \cite{tschannen_autoproof:_2015} --- a verifier for Eiffel ---, to detect lack of consistency in the system. In this paper, the author also propose to directly link requirements expressed in different formalisms (natural language, diagram) inside the programming code. This approach should help user to find informations about the source of a piece of the program, and to make traceability from specification to realization.

% Need to cite works of A. Naumchev

\subsection{Traceability and multirequirements}

According to the \gls{INCOSE} \cite{incose_se_????}, another important concern on system engineering is the traceability issue. Indeed, due to the iterative add of requirements in  life cycle of a complex system project, the traceability notion is required to evaluate the change impact. We can distinguish two kinds of traceability: 
\begin{itemize}
  \item a requirement/requirement traceability, useful to determine what other requirements are concerned by a change and to understend links between requirements (e.g., the composition, "refine", "derive", etc. links in \gls{SysML});
  \item a requirement/design traceability, useful to determine the part of a system impacted by change and which requirement is fulfilled by the implementation (e.g., the multirequirements viewpoint in \cite{meyer_multirequirements_2013} --- the "satisfy" link in \gls{SysML}).
\end{itemize}

In \cite{soares_user_2011}, Soares et al. propose to extend SysML to provide a better structured way to express requirements. By adding explicit relationship between requirements, especially in requirements table, they improve the traceability notion in requirements expression, making explicit (and semantically defined via metamodel) links between requirements. Indeed, they highlight that the type of relation existing between requirements is important to measure the impact change. However, in this paper, the solution proposed still require the human expertise to determine the change effect.

Similarly, Albinet et al. \cite{albinet_memvatex_2008} propose a methodology based on \gls{EAST-ADL2}, \gls{SysML} and \gls{MARTE} \cite{object_management_group_omg_marte_2011} --- a \gls{UML} profile for real-time and embedded applications. They enrich these languages, in order to keep the idea of traceability between requirements and components proposed by \gls{SysML}, while they use notions of \gls{MARTE} to complete \gls{EAST-ADL2} --- a language to design automotive systems. However, this approach is domain-centric (automotive embedded systems) and must be globalized to other models.

In a requirement/design traceability approach, work from Meyer \cite{meyer_multirequirements_2013} also proposed a way to link specification and implementation. Indeed, by proposing to use a unique language, Eiffel, to express requirements --- combining specification in natural language, with diagrams, with design by contracts ---, the author enables to directly link requirement with their implementation, allowing to easily trace requirements. However, though this approach can be applied to software engineering, system engineering does not use the classes paradigm to model systems, and a parallel between standard system engineering representation and object oriented paradigm should be explored. 

\section{Goal of the Project}

To allow the introduction of seamlessness in complex system, a number of research leads must be explored. Indeed, in order to produce a methodology and tools that can be used in a real industrial context, our contributions should be easy to handle and as close as possible to languages and tools used by engineers.

The main goal of our project are:
\begin{itemize}
  \item to specify a common interface (as a language or a metamodel) to link artifacts of different domains, with a defined formal semantic to be able to express existing relationships between specification from several stakeholder (a multiviews approach);
  \item to define links between this requirement interface and the system, in order to provide a backward and forward traceabilities (a multirequirements approach);
  \item to provide tools, based on this interface, in order to assist requirements engineers in controlling the consistency, ensuring the system validity.
\end{itemize}

In order to validate our contribution, we expect to apply our methodology on an industrial real-case example.

\subsection{Multiviews}
\label{sec:goal-multiviews}

Existing approaches to express requirements are not widely used. This gap of acceptance is probably due to the force of habits which slows engineers to adopt these new techniques. Another difficulty is the lack of support for verification and validation, either at requirements level or at traceability level. We expect to provide tools that can be interfaced with usual tools, in order to ease adoption of a new methodology. A number of locks however remain, and even if \gls{MBSE} approach seems to provide a framework, we should define a modeling as close as possible to reality. Indeed, the use of \gls{MDE} should permit us to make links between different stakeholders (existing metamodels of their formalism --- or deduced metamodels --- can easily be transform to a new metamodel). However, we have to provide a language that is the more complete possible, especially in term of relationship, if we do not want a loss of information during transformation. Hence we have defined a set of research questions.

\subsubsection{Research questions}
\begin{itemize}
  \item How to express the requirements so that remain human readable but can also be interpreted by a computer?
  \item What are the essential characteristics of a requirement?
  \item What kind of requirements are existing and which links do exist between them?
  \item How to use this formalization to prove properties of the requirements systems?
  \item How to link artifacts from several stakeholders?
\end{itemize}

\subsubsection{Research methods}
\begin{itemize}
  \item Define a requirements language (syntax and semantic) based on main characteristics of requirements according to state-of-the-art;
  \item Use a constraint language as a back-end engine to infer formal properties of requirements;
  \item Study of existing tools and standards in order to deduce syntax so that we can use them in coordination with our language;
  \item Provide a language that can be used as an interface between specifications of different stakeholders;
  \item Define strongly semantically relationship between requirements in order to provide traceability between several stakeholders.
\end{itemize}

\subsubsection{Expected contributions}
\begin{itemize}
  \item A new interface way of requirements systems expressed in different languages coming from different domains (e.g., use of a common metamodel, use of existing globalization framework such as \gls{GEMOC} \cite{combemale_globalizing_2014}, etc.);
  \item A formal method to infer some properties of requirements, based on a constraint language;
  \item A traceability tool, able to clearly point what are the artifacts impacted by a change in the system.
\end{itemize}

\subsection{Multirequirements}

Another major issue in complex system engineering is the traceability between specification and realization. If the link may seem to be easy to do in software engineering, especially with \gls{MDE} approach that can provide a common artifact --- models --- to specify and to implement the system, in the system engineering case, with some real hardware component, the problem is harder. The \gls{MBSE}, by advocating the use of models as a central artifact in the development of complex system, provides an entry point to solve this problem. Indeed, nowadays this approach is widely used, and from the specification to simulation, models are a corner stone. Linked to our previous problematic, we expect to express specification as models and, if systems are also expressed with these artifacts, make a backward and forward traceability should be widely supported. To contribute to this issue, we have identified a set of research questions. 

\subsubsection{Research questions}
\begin{itemize}
  \item How to link specification with system realization?
  \item What is the semantic behind these links?
  \item How to deduce requirements from the system design itself?
  \item Are we able to propose some valid logical solutions (that satisfy the requirements) from specification (e.g., as we did in \cite{galinier_algorithmes_2016})?
\end{itemize}

\subsubsection{Research methods}
\begin{itemize}
  \item Enrich the language mentioned in \ref{sec:goal-multiviews} to group system definition and specification in a same formalism;
  \item Explore verification and validation tools (such as theorem provers) and simulation tools as supports for the semantic of links between requirements and design artifacts;
  \item Make strong link between specification and realization artifact, in order to be able to navigate from one to the other in both directions.
\end{itemize}

\subsubsection{Expected contributions}
\begin{itemize}
  \item An operational semantic for our requirements language;
  \item A multirequirement approach, based on software existing ones;
  \item An integrated tooling support (e.g., in Eiffel as a proof of concept, in Eclipse for industrial collaboration support) that can be used to assist requirements engineers to check (possibly by construction) the correctness of the ongoing design of the system.
\end{itemize}

\section{Detailed Work Plan}

We have defined a number of task to carry out this project, enumerate below. The provisional planning is given in the Gantt chart, fig. \ref{fig:gantt}.

\subsubsection{Formalization of requirements}
\begin{enumerate}[label=(\arabic*)]
  \item Define a common language interface for requirements and systems.
  \item Formalize requirements, based on their main characteristics and provide interface with existing used ones.
  \item Make the link between our interface and the backend language.
\end{enumerate}

\subsubsection{Apply to real case example}
\begin{enumerate}[label=(\arabic*),resume]
  \item Find and apply our approach on a case study.
  \item Validate by stressing out our approach to a number of realistic projects. 
\end{enumerate}

\subsubsection{Final thesis redaction}
\begin{enumerate}[label=(\arabic*),resume]
  \item Focus on the redaction of thesis document
\end{enumerate}


\begin{landscape}
\vspace*{\fill}
\begin{figure}[h!]
\centering
\begin{tikzpicture}
\begin{ganttchart}[y unit title=0.7cm,
y unit chart=0.8cm,
vgrid,hgrid, 
title label anchor/.style={below=-1.6ex},
title left shift=0,
title right shift=0,
title height=1,
bar/.style={fill=gray!50},
incomplete/.style={fill=white},
progress label text={},
bar height=0.7,
group right shift=0,
group top shift=0.3,
group height=0.7]{1}{36}
%labels
\gantttitle{2016}{3}
\gantttitle{2017}{12} 
\gantttitle{2018}{12} 
\gantttitle{2019}{9} \\
\gantttitlelist{10,...,12}{1} 
\gantttitlelist{1,...,12}{1} 
\gantttitlelist{1,...,12}{1} 
\gantttitlelist{1,...,9}{1} \\
%tasks
\ganttgroup{Formalization of requirements}{1}{32} \\
\ganttbar{Multirequirements (1)}{1}{24} \\
\ganttbar{Multiviews (2)}{12}{32} \\
\ganttbar{Link with backend language (3)}{3}{32} \\
\ganttgroup{Apply to example}{3}{33} \\
\ganttbar{Apply on a case study (4)}{3}{22} \\
\ganttbar{Stress out with realistic projects (5)}{22}{33} \\
\ganttgroup{Final thesis redaction}{30}{36} \\
\ganttbar{Focus on thesis redaction (6)}{30}{36}
\end{ganttchart}
\end{tikzpicture}
\caption{\label{fig:gantt}Forecast Gantt chart of project}
\end{figure}
\vspace*{\fill}
\end{landscape}


==> notes/trace.tex <==
% \section{Using relational model transformations to reduce complexity in {SoS} requirements traceability: {Preliminary} investigation \cite{dickerson_using_2010}}
% \setcounter{MaxMatrixCols}{20}
%
% Document Centric to Model Centric engineering
%
% Dependence Structure Matrix (matrix $A(x,x) | x \in \mathbb{N}$ where $\forall x,y \in artifacts, A(x,y) = true$ iff there is a relation between artifacts $x$ and $y$.
% Problem: Cannot link through several artifacts
%
% Relational transformation using matrix
% \begin{align*}
% \begin{matrix}
%    &    &    &    &    &    &    &    &    &    & x1 \\
%    &    &    &    &    &    &    & \cmark & \cmark &    & x2 \\
%    &    &    &    &    &    & \cmark &    &    & \cmark & x3 \\
%    &    &    &    &    &    &    &    &    &    & x4 \\
%    &    &    &    &    &    &    & \cmark & \cmark &    & x5 \\
% y1 & y2 & y3 & y4 &    & x1 & x2 & x3 & x4 & x5 & \\
%    &    &    &    & y1 &    &    &    &    &    & \\
%    &    & \cmark & \cmark & y2 & & \cmark & & & \cmark & \\
%    & \cmark & & & y3 & & & \cmark & & & \\
%    & & & & y4 & & & & \cmark & & \\
% \end{matrix}
% \end{align*}
%
\section{Model-based requirements engineering for system of systems \cite{holt_model-based_2012}}

In this work, the authors propose an \gls{ACRE} ontology for requirements to link them to system of system. They define a metamodel that introduce link between requirements and a context. There are the uses cases that act to describe a scenario in a particular context apply to requirements; that permits to simply infer validation scenarios to test the satisfaction of requirements.

However, the issue in our opinion of a such approach is that there is no direct link with concrete system elements but, due to the fact that requirements are associated with a context, the requirements are link with complete systems.
In a \gls{SoS} case, systems are part of a more complex system and can be considered as elements, but it stays very specific.

In their work, the authors also provide several views for requirements engineers to analyze the system. They especially conserve a link between requirements and sources of them (from where the requirements were elicited), allowing a traceability from the beginning of the requirements process. 

% TODO: Rephrase this review
% \section{A {Survey} of {Traceability} in {Requirements} {Engineering} and {Model}-driven {Development} \cite{winkler_survey_2010}}
%
% \begin{quotation}
%   Traceability between artifacts that are not necessary requirements (useful in our project?)
% In this context, Traceability is defined in the IEEE Standard Glossary of Software Engineering Terminology [90] as
% 1.  The degree to which a relationship can be established between two or more products of the development process, especially products having a predecessor–successor  or  master–subordinate relationship to one another. [...]
% 2.  The degree to which each element in a software development product establishes its reason for existing.
% \end{quotation}
%
% According to Gotel and Finkelstein (RE'94), traces should also be applied to requirements modifications (during refinement process).
%
% In our opinion, at least a subset of traceability links should be expressed in requirements expression; indeed, as requirements are defined by these links, it seems logical to model traceability links in a metamodel that should defined a requirement.
%
\section{The {Single} {Model} {Principle} \cite{paige_single_2001}}

In this paper, the authors propose the base of the multirequirements approach proposed by Meyer in \cite{meyer_multirequirements_2013}. They argue that in \gls{UML} link to Java language, even if it exists links between models, they are several models to describe a system, contrary to Eiffel with \gls{BON}, where the different abstraction of a system can be expressed in a single model, reducing the gap between modeling representation and implementation. Their opinion is based on the metamodels of \gls{UML} and \gls{BON}, that organize \texttt{Model} elements in different ways; in \gls{UML}, \texttt{Model} is an element like other while in \gls{BON}, \texttt{Model} is composed by the several abstractions. However, it is important to note that this article was wrote in 2001, with an older version of \gls{UML}.

According to Paige and Ostroff, the introduction of requirements in the modeling language can lead to link them to concrete elements. However, even if they exists requirements modeling language (such as the KAOS \gls{GORE} approach), they are not included in the BON/Eiffel system and so, introduction of these notions will break the single model principle. They propose to use an intermediate transformation (from KAOS to Z and from Z to Eiffel) to introduce requirements in Eiffel; nevertheless, it will not have traceability links from requirements to their source.

This approach of Single Model Principle described for Software Engineering here can lead us to create our multirequirements approach for System Engineering. According to authors, they are several important points to respect this principle: 
\begin{itemize}
  \item all phases (from requirements to specification and from specification to implementation) must be expressed in a single modeling language;
  \item they must be an only models that groups all abstractions and not several views, each one used to describe a part of systems.
\end{itemize}

\section{KAOS to \gls{UML}/\gls{OCL}}

There are a lot of works that treat the transformation from KAOS to \gls{UML}. In \cite{chanvilai_goal-oriented_2012}, the authors propose an approach to model in \gls{UML} the goals and requirements expressed with KAOS. They also propose transformation of functional requirements in \gls{OCL}; however, this stays a manual transformation and, according to the authors, most of the requirements cannot be expressed in \gls{OCL} due to the fact that KAOS owns temporal elements that are not available in \gls{OCL}.

A previous work try to treat this issue. In \cite{robinson_extended_2007}, the authors propose an extension of \gls{OCL}, named $OCL_{TM}$ (for \gls{OCL} with Temporal Message). Their approach aims to provide a language to express requirements directly in models, arguing that \gls{OCL} users base is larger than KAOS one. However, even if this works allow a better expression for requirements with introduction of temporal elements, the \gls{OCL} syntax makes it difficult to understand for non-software engineers.

\section{Testable {Requirements} and {Specifications} \cite{ostroff_testable_2007}}

In this paper, Ostroff and Torshizi propose to introduce requirements in \gls{BON}/Eiffel to apply the approach of Single Model Principle \cite{paige_single_2001} previously mentioned. They propose the use of a framework to make requirements testable. They propose two approaches:
\begin{itemize}
  \item the first one consists on a translation from requirements express in tables to Eiffel language as scenario tests. This can be assimilate to the expression of requirements in the form of behavioral models such as sequence diagrams or state diagram.
  \item the second one consists on a translation of some requirements as contracts of the Eiffel source code.
\end{itemize}

These approaches permit during description of the system to detect lack of consistency. They categorized two kind of errors:
\begin{itemize}
  \item design errors,
  \item and implementation errors.
\end{itemize}
Their two approaches allows to detect these two kind of errors, than can be rely to detect if this is the wrong system (design errors) or if the system is wrong (implementation errors).
One of the main objective of this thesis is to assist requirements engineers, and the \gls{VV} analysis --- that consists to detect these kind of errors --- is an important part of their work.

The main issue of this approach in our opinion is that there is clearly software specific and need the intervention of a developer to link requirements (scenarios tests or contracts) and the architecture. Furthermore, even if the authors stick to the Single Model Principle, in our opinion the requirements' sources must also be included in this single model, that is not done with their approach.

\section{{fSysML}: {Foundational} {Executable} {SysML} for {Cyber}-{Physical} {System} {Modeling} \cite{badreddin_fsysml:_2016}}

In this work, the authors propose a executable language subset of \gls{SysML} for \gls{CPS}. Their objective is to provide a more convenient and portable way to express models. This language especially permit the expression of goals and soft-goals (which are requirements) and to link them with other more common \gls{SysML} elements, such as behavioral specification or blocks definition. The authors inter alia argue that the semantic on links involving requirements have to be stronger defined, links such as \emph{satisfy} or \emph{verify} links must have implications in testing and analysis phases. Furthermore, in their language they introduce some semantic on links between requirements that does not exists in \gls{SysML} -- especially the idea of contribution of a subgoal to the goal that is composed by this subgoal.

The use of a textual language is moreover important for versioning the evolution of system. Indeed, in \gls{RE}, traceability across elements is crucial to detect inconsistency, but traceability across time is also important to analyze when change were introduced in the system. A textual language is for that purpose more convenient.

In our opinion, the need for semantic on requirements also need to be introduce in their expression; in this paper, authors introduce some notions that can be interested to use to define a more formal way to express requirements.


==> surveyTable.tex <==
\begin{table}[hbt] 
\centering
    \begin{tabular}{cl*{10}c}
        & \rot{Readability} & \rot{Meth. independence} 
        & \rot{Traceability} & \rot{Formal definition} & \rot{Metadata} 
        & \rot{\textbf{O}perational/\textbf{D}enotational} &  \rot{Category (cf. \mysec{approaches}.)} \\ 
       %\cmidrule{2-12}
%--- General purpose
IBM Rational Doors & \OK & \OK & \OK & \NOK & \OK & D & G \\ 
KAOS & \OK & \OK & \OK & \NOK & \NOK & D  & G \\ 
Reqtify & \OK & \OK & \OK & \NOK & \OK & O &  G \\ 
SysML & \OK & \OK & \OK & \OK & \OK & D  & G \\ 
URML & \OK & \OK & \OK & \NOK & \NOK & D  & G \\ 
URN & \OK & \OK & \OK & \NOK & \NOK & D  & G \\ 
%--- Natural language
NLtoOCL & \OK & \NOK & \OK & \OK & \NOK & O  & N \\ 
NLtoOWL & \NOK & \OK & \OK & \OK & \NOK & D & N \\ 
NLtoSTD & \OK & \OK & \NOK & \OK & \NOK & D & N \\ 
Relax & \OK & \OK & \NOK & \OK & \NOK & D & N \\ 
Requirements grammar & \OK & \OK & \NOK & \NOK & \NOK & D  & N \\ 
%--- Graph and Automata
FORM-L & \NOK & \OK & \OK & \OK & \OK & D  & A \\ 
LTSA & \NOK & \OK & \NOK & \OK & \NOK & O   & A \\ 
Petri Nets & \OK & \OK & \NOK & \OK  & \NOK & O  & A \\ 
Problem Frames & \OK & \OK & \NOK & \NOK & \NOK & D & A \\ 
Statecharts & \OK & \OK & \NOK & \OK & \NOK & O  & A \\ 
%--- Mathematical notation
Alloy & \NOK & \OK & \OK & \OK & \NOK & D  & M \\ 
Event-B & \NOK & \OK & \OK & \OK & \NOK & O & M \\ 
Process Algebra & \NOK & \OK & \NOK & \OK & \NOK & O  & M \\ 
VDM & \NOK & \OK & \OK & \OK & \NOK & D   & M \\ 
%--- Programming Language
Multirequirements & \OK & \NOK & \OK & \OK & \OK  & O & P \\ 
       % \cmidrule[1pt]{2-12}
\end{tabular}
\caption{Overview of the approaches evaluation}
\label{tab:results}
\end{table}
%\fg{Is there a reason for the 'N' in the Formal definition column for statecharts?} => corrected by JMB

%\TODO{center the fig (remove the 1st empty column)}

